Weighted Connected Matchings

A matching $M$ is a $\mathscr{P}$-matching if the subgraph induced by the endpoints of the edges of $M$ satisfies property $\mathscr{P}$. As examples, for appropriate choices of $\mathscr{P}$, the problems Induced Matching, Uniquely Restricted Matching, Connected Matching and Disconnected Matching arise. For many of these problems, finding a maximum $\mathscr{P}$-matching is a knowingly NP-Hard problem, with few exceptions, such as connected matchings, which has the same time complexity as usual Maximum Matching problem. The weighted variant of Maximum Matching has been studied for decades, with many applications, including the well-known Assignment problem. Motivated by this fact, in addition to some recent researches in weighted versions of acyclic and induced matchings, we study the Maximum Weight Connected Matching. In this problem, we want to find a matching $M$ such that the endpoint vertices of its edges induce a connected subgraph and the sum of the edge weights of $M$ is maximum. Unlike the unweighted Connected Matching problem, which is in P for general graphs, we show that Maximum Weight Connected Matching is NP-Hard even for bounded diameter bipartite graphs, starlike graphs, planar bipartite, and bounded degree planar graphs, while solvable in linear time for trees and subcubic graphs. When we restrict edge weights to be non negative only, we show that the problem turns to be polynomially solvable for chordal graphs, while it remains NP-Hard for most of the cases when weights can be negative. Our final contributions are on parameterized complexity. On the positive side, we present a single exponential time algorithm when parameterized by treewidth. In terms of kernelization, we show that, even when restricted to binary weights, Weighted Connected Matching does not admit a polynomial kernel when parameterized by vertex cover under standard complexity-theoretical hypotheses.

==> appendices.tex <==
\newpage
\setcounter{section}{0}
\renewcommand\thesection{\Alph{section}}
\section*{Appendix}

\section{Proof of Theorem ...}


==> wcs.tex <==
\section{Weighted Connected Subgraph}

\nproblem{Weighted Connected Subgraph}{A graph $G=(V,E)$ and an integer $k$}{Is there a set $V' \subseteq V$ such that the sum of the weights of the vertices of $V'$ is at least $k$ and $G[V']$ is connected?}

Uma redução de prize-collecting Steiner tree https://www.ncbi.nlm.nih.gov/pmc/articles/PMC2718639/pdf/btn161.pdf
https://dimacs11.zib.de/workshop/ElKebirKlau.pdf

The optimization problem 
{ \sc Maximum-Weight Connected Subgraph }(MWCS) is widely studied by the heuristic and optimization community\textcolor{red}{referências}. Besides the contribution to the optimization field, some also have shown relevant computational complexity results. One example is the hardness proof of an approximation algorithm in~\cite{mwcs_approx_hardness}.

However, a lot of papers rely on complexity results that are not easily accessible. In particular, we could not find any proof showing explicitly the {\NPcness} proof for bipartite, planar, bounded diameter or bounded maximum vertex degree, though widely referenced.

One of the references presented by many articles is a manuscript~\cite{vergis}, which is used when referring to the {\NPcness} of {\sc Maximum-Weight Connected Subgraph } for planar graphs with bounded maximum vertex degree and vertex weights $-1$ or $+1$. Yet, we had no success in finding any way to access this content.

With this same difficulty, other scientists asked about this proof, which motivated Marzio De Biasi to rewrite the proof by himself in 2014 in StackExchange~\cite{marzio_de_biasi}. The concepts he presented for the {\NPcness} were solid, though it was not formally wrote in a paper. In Section~\ref{sec:wcs-planar}, we use his reduction, with little modifications, in order to prove the {\NPcness} of {\sc Weight Connected Subgraph } even for planar graphs with maximum vertex degree at most three and vertex weights $-1$ or $+1$. This is exactly the result obtained by Vergis~\cite{vergis}. So, with this proof

Another successful attempt, due the lackness of formal {\NPc} proofs, was done by Benno Schwikowski in 2002~\cite{benno_schwikowski}. He wrote by himself a sketch of the {\NPHness} proof for the {\sc Maximum Weight Connected Subgraph}, provided by Richard M. Karp. This reduction is interesting and compliments the previous results, as it proves {\NPHness} for bipartite graphs with bounded diameter at most $4$. In Section~\ref{sec:wcs-bipartite}, we formally wrote this proof, showing some more details and an example.

For Sections~\ref{sec:wcs-planar} and ~\ref{sec:wcs-bipartite}, we restrict the proofs to the {\NPHness}, since the pertinence into {\NP} is simpler and can be shown once and separately, as shown in Lemma~\ref{wcs-np}.

\begin{lemma}\label{wcs-np}
{\sc Weighted Connected Subgraph} is in {\NP}
\end{lemma}\label{lemma:wcs-np}
\begin{proof}
Let $V' \subseteq V(G)$ be a certificate for the answer {\YES} such that $G[V']$ is connected and whose vertices weights sum is at least $k$. To validate $V'$, all we need is to verify that $G[V']$ is connected and the sum of the weights of $V'$ is indeed at least $k$, which can be done in polynomial time. So, the problem is in {\NP}.
\end{proof}

\subsection{{\sc Weighted Connected Subgraph } for bipartite graphs}\label{sec:wcs-bipartite}

In this section, we show the {\NPcness} of the {\sc Weighted Connected Subgraph} even for bipartite graphs with diameter at most four.

The {\NPHness} proof is obtained using a reduction from the well known {\NPc} problem {\sc Set Cover}~\cite{karp_72}.

\nproblem{Set Cover}{A set $U$, a collection $S$ of sets whose union equals $U$, and an integer $k$}{Is there a collection $S' \subseteq S$ whose union equals $U$ and the cardinality of $S'$ is at most $k$.}

For the following reduction, we assume that there is no empty set as an element of $S$, because, if it had, we could remove those sets from $S$ with no loss. Also, every element of $U$ must be contained in at least one set of $S$; otherwise the answer would be {\NOi}.

Let $k'$, $U$ and $S$ be an input for { \sc Set Cover }, and $q = |U|$ and $p = |S|$. For the { \sc Weighted Connected Subgraph } input, we set $k = (q+1)(p+1)-k'$.

\begin{enumerate}[(I)]
    \item For each set $T$ of $C$, add a vertex $c_T$ such that $weight(c_s) = -1$
    \item For each element $u$ of $U$, add a vertex $s_u$, such that $weight(s_u) = q+1$, and the edges $s_uc_t$ for every set $t \in S$ that contains the element $u$
    \item Add a vertex $h$, such that $weight(h) = q+1$, and the edge $hc_s$ for every set $s \in S$ 
\end{enumerate}

The goal with this transformation is that, to be able to have a satisfying $V'$, then $h$ and every vertex $s_u$, $u \in U$, must be contained in $V'$. Otherwise, $V'$ wouldn't reach it's desired value. Moreover, inside $V'$, there can be at most $k$ vertices from $\{ c_u \mid u \in S \}$.

If such set $V'$ exists, it means that, for every element $u \in U$, there is a vertex $c_t$, $t \in S$, such that $u \in c_t$. Thereby, those vertices $c_t$ represent the sets that corresponds to a solution of {\sc Set Cover}.

Note that, $G$ is indeed bipartite as the two sets of independent vertices can be $\{ c_i \mid i \in S \}$ and $\{ h \} \cup \{ s_i \mid i \in U \}$.

Also, the graph has diameter at most $4$. This is due to the distance of two vertices, $s_x$ and $s_y$, such that there is no set $t \in S$ that contains both $x$ and $y$. For this reason, a shortest path between $s_x$ and $s_y$ must contain $h$ and two vertices related to sets such that each contains eather $x$ or $y$. 

\begin{lemma}\label{lemma:wcs-1-ida}
Let $(U,S,k')$ be an input of {\sc Set Cover }, $S'$ be a solution of this instance, and $G$ be the transformation graph obtained from this input. A set $V' \subseteq V(G)$ such that $|V'| = (q+1)(p+1) - k'$ and $G[V']$ is connected can be obtained in polynomial time.
\end{lemma}
\begin{proof}

\end{proof}

\begin{lemma}\label{lemma:wcs-1-vvolta}
Let $(U,S,k')$ be an input of {\sc Set Cover } and $G$ be the transformation graph obtained from this input. Given a set $V' \subseteq V(G)$ such that $|V'| = (q+1)(p+1) - k'$ and $G[V']$ is connected, a solution $S'$ for the {\sc Set Cover } instance can be obtained in polynomial time.
\end{lemma}
\begin{proof}

\end{proof}

Then, we present Theorem~\ref{teo:wcs-bipartite} as our final result for the problem in bipartite graphs.

\begin{theorem}
{\sc Weighted Connected Subgraph} is {\NPc} even for bipartite graphs with diameter at most $4$
\end{theorem}\label{teo:wcs-bipartite}
\begin{proof}
Lemma~\ref{lemma:wcs-np} shows that the problem is in {\NP}. Next, we demonstrate that it is {\NPH}.
\end{proof}

\subsection{Example}

Let's consider the input for {\sc Set Cover } defined as $k'=2$ and $U = \{ a,b,c,d,e,f,g \}$, $S = \{ T,W,X,Y,Z \}$, as $T = \{ a,b,e \}$, $W = \{ a,b,c,d \}$, $X = \{ c,f \}$, $Y = \{ e,f,g \}$, $Z = \{ d \}$; in other words, $S = \{ \{ a,b,e \}, \{ a,b,c,d \} , \{ c,f \}, \{ e,f,g \}, \{ d \} \}$. Then, our reduction for {\sc Weighted Connected Subgraph } is $k = 8\cdot6-2 = 46$ and the graph ilustrated in Figure~\ref{fig:wcs-red-1}.

In this case, the solution for in {\sc Weighted Connected Subgraph} is $V' = \{ h, s_a, s_b, s_c, s_d, s_e, s_f, s_g, c_W, c_Y \}$, in which the sum of the vertex weights is exactly $46$. For {\sc Set Cover}, this corresponds to the solution $S' = \{ W, Y \}$, as $c_W$ and $c_Y$ are saturated.

\begin{figure}
    \centering
    \includesvg[width=1\textwidth]{images/svg/emp-conexo-pond-red-example}
    \caption{Example of a reduction graph for {\sc Set Cover}}
    \label{fig:wcs-red-1}
\end{figure}


\subsection{{\sc Weighted Connected Subgraph } for planar graphs}\label{sec:wcs-planar}



%Instance: an undirected graph $G=(V,E)$, a subset of the vertices $R \subseteq V$, a non-negative integer $k$
%Question: is there a subtree of G that includes all the vertices of $R$ (a spanning tree for $R$) and that contains at most $k$ edges?

In this section, we prove the {\NPcness} of {\sc Weighted Connected Subgraph} even for planar graphs with maximum vertex degree three and vertex weights $-1$ or $+1$. For this purpose, we use one of the Karp's original $21$ {\NPc} problems, the {\sc Steiner Tree}~\cite{karp_72}, which is described in the following.

\nproblem{Steiner Tree}{A graph $G=(V,E)$, a subset of the vertices $R \subseteq V$, a non-negative integer $k$}{Is there a subgraph $T$ of $G$ such that $T$ is a tree and includes all the vertices of $R$ and that contains at most $k$ edges?}

Garey and Johnson showed in~\cite{rectilinear_steiner_tree} that this problem is {\NPc} even for planar graphs, as they showed the {\NPcness} for {\sc Rectilinear Steiner Tree}. Thereby, we can make our reduction using the {\sc Steiner Tree}, even if we restrict the input graph to be planar.

Let $(G', R, k')$ be an input of { \sc Steiner Tree} restricted to planar graphs.

\begin{align*}
&q = \Delta(G') \\
&p = q(|V| - |R|) + 1 \\
&r = p|E| + 1
\end{align*}

For our reduction to { \sc Weighted Connected Subgraph } input, we set $k = r|R| - pk'$ and the input
graph $G$ built with the following procedures.

\begin{enumerate}[(I)]
    \item For each vertex $w$ add a copy of a cycle graph with length $r$ if $w \in R$, and $q$ otherwise. If this length is less then $3$, instead, add a copy of a path graph with the same number of vertices as the intended cycle length. Set the weights of all these vertices as $+1$. Besides, add the label for $|N(w)|$ of these vertices as $v_{wu}$, for each $u \in N(w)$. 
    %Add the label for the remaining $i$ non-labeled vertices as $v_{w1},\ldots,v_{wi}$.

    \item For each edge $wu$ in $E$, generate a copy of $P_{p}$ whose vertex weights are $-1$ and make its terminal vertices disjointly adjacent to $v_{wu}$ and $v_{uw}$.
\end{enumerate}

The goal of this transformation is that all the vertices of the subgraphs generated by vertices of $R$ must be contained in $V'$, as their weight is big enough. Also, at most $k$ paths, generated by edges of $G'$, are allowed to be in $V'$; otherwise it would be impossible to reach the desired weight sum. The weights from vertices of the subgraphs generated by $R \setminus V$ are irrelevant, because, even if all are in $V'$, they increase the weight sum by a small value.

First, we show in Lemma~\ref{lemma:wcs-planarity} that the transformation graph keeps the planarity of the original input graph. This is fundamental to our proof, since we want to show the {\NPcness} of {\sc Weighted Connected Subgraph } even for planar graphs.

Besides, the transformation graph has three as the maximum vertex degree. This is due to the transformation procedure in (I). It is worth mentioning that the technique of adding cycles whose lengths is greater than $\Delta(G)$  was also used in a {\NPcness} proof of {\sc Vertex Cover } for planar graphs with maximum vertex degree three~\cite{rectilinear_steiner_tree} .

\begin{lemma}\label{lemma:wcs-planarity}
Let $G'$ be any input graph for {\sc Steiner Tree} and $G$ its transformation graph for {\sc Weighted Connected Subgraph}, as described below. The maximum degree of $G$ is three and, if $G'$ is planar, then $G$ is also planar.
\end{lemma}
\begin{proof}
There are two main modifications

(I) Add of a cycle.

(II) Add vertices in an edge
Both modifications doesn't make any difference in terms of planarity. So, if $G'$ is planar, then $G$ has also this property.
\end{proof}

\begin{figure}
    \centering
    \includesvg[width=0.6\textwidth]{images/svg/emp-conexo-pond-red-1-example-2-1}
    \caption{Example of a representation of a reduction graph for {\sc Steiner Tree}}
    \label{fig:wcs-red-2-1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{images/emp-conexo-pond-red-1-example-2-2.png}
    \caption{Example of a representation of a reduction graph for {\sc Steiner Tree}}
    \label{fig:wcs-red-2-2}
\end{figure}

\begin{lemma}\label{lemma:wcs-planarity}
Let $G'$ be any input graph for {\sc Steiner Tree} and $G$ its transformation graph for {\sc Weighted Connected Subgraph}, as described below. If $G'$ is planar, then $G$ is also planar.
\end{lemma}
\begin{proof}
\end{proof}

Now we show that ...............


\begin{lemma}\label{lemma:wcs-1-ida}
Let $(G',R,k')$ be an input of {\sc Steiner Tree }, $T$ be a solution of this instance, and $G$ be the transformation graph obtained from this input. Consider $q = \Delta(G')$, $p = q(|V| - |R|) + 1$ and $r = p|E| + 1$. A set $V' \subseteq V(G)$ can be obtained in polynomial time such that $|V'| = r|R| - pk'$ and $G[V']$ is connected.
\end{lemma}
\begin{proof}

\end{proof}

\begin{lemma}\label{lemma:wcs-1-vvolta}
Let $(G',R,k')$ be an input of {\sc Steiner Tree }, and $G$ be the transformation graph obtained from this input. Consider $q = \Delta(G')$, $p = q(|V(G')| - |R|) + 1$ and $r = p\cdot|E(G')| + 1$. Given a set $V' \subseteq V(G)$ such that $|V'| = r|R| - pk'$ and $G[V']$ is connected, a solution $T$ for the {\sc Steiner Tree } instance can be obtained in polynomial time.
\end{lemma}
\begin{proof}

\end{proof}

\begin{theorem}
{\sc Weighted Connected Subgraph} is {\NPc} even for planar graphs with maximum vertex degree $3$ and its vertex weights in $\{ -1, +1 \}$
\end{theorem}\label{teo:wcs-planar}
\begin{proof}
Lemma~\ref{lemma:wcs-np} shows that the problem is in {\NP}. Next, we shot that it is {\NPH}. In the following, we prove that it is also {\NPH}.
\end{proof}

\subsection{Example 1}

We consider the input for {\sc Steiner Tree} as $k' = 1$, $R = \{ a,b \}$ and the graph $G'$ isomorphic to $C_3$, with $V(G') = \{ a,b,c \}$.

In this case we have the following variable values.

\begin{align*}
&q = \Delta(G') = 2 \\
&p = q(|V| - |R|) + 1 = 3 \\
&r = p|E| + 1 = 10
\end{align*}

So, for the {\sc Weighted Connected Subgraph} input, we set $k = 17$, and the graph as the one illustrated in Figure~\ref{fig:wcs-red-1-2}.

To solve {\sc Weighted Connected Subgraph} for this instance, we need to find $V' \subseteq V$ such that $G[V']$ is connected and the sum of its vertex weights is at least $17$.

To reach this value, $V'$ must contain vertices of each of the $C_{10}$ subgraphs, which were generated because of $a$ and $b$ of $G'$. Observe that there is no loss in adding all the $20$ vertices of these subgraphs in $V'$, so we can increase the weights sum by that. In consequence of $G[V']$ being connected, there must be a path between the $C_{10}$ subgraphs contained in $V'$. Note that there is only two possible paths of these, one with length $9$, between $v_{ac}$ and $v_{bc}$, and other with length $4$, between $v_{ab}$ and $v_{ba}$. The vertex weights sum for this first path is $-4$ and, for the second, $-3$.

Then, we can conclude that the only possible vertex set $V'$ includes this path between $v_{ab}$ and $v_{ba}$ and all the $20$ vertices of the $C_{10}$ subgraphs. This solution is shown in bold in Figure~\ref{fig:emp-conexo-pond-red-1-example-1-2} and corresponds to the {\sc Steiner Tree} solution $G[\{a,b\}]$.

\begin{comment}
\begin{figure}
    \centering
    \includesvg[width=0.2\textwidth]{images/svg/emp-conexo-pond-red-1-example-1-1}
    \caption{Example of a representation of a reduction graph for {\sc Steiner Tree}}
    \label{fig:emp-conexo-pond-red-1-example-1-1}
\end{figure}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{images/emp-conexo-pond-red-1-example-1-2.png}
    \caption{Example of a reduction graph for {\sc Steiner Tree}}
    \label{fig:emp-conexo-pond-red-1-example-1-2}
\end{figure}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{images/eps/wcm-planar-example}
    \caption{Example of a \pname{Weighted Connected Matching} reduction for the Figure \ref{fig:emp-conexo-pond-red-1-example-1-2} graph}
    \label{fig:wcm-planar-example}
\end{figure}
\end{comment}

\subsection{Example 2}

We consider the input for {\sc Steiner Tree} as $k' = 3$, $R = \{ a,c,d \}$ and the graph $G'$ as in Figure~\ref{fig:wcs-red-2-1}. In this case we have the following variable values.

\begin{align*}
&q = \Delta(G') = 4 \\
&p = q(|V| - |R|) + 1 = 13 \\
&r = p|E| + 1 = 105
\end{align*}

The transformation subgraph is shown in Figure~\ref{fig:wcs-red-2-2}. For a better visualization, we denote the subgraph $P_p$ by a square. Each of its edges are incident to terminal vertices of $P_p$. Also, a triangle represents a cycle subgraph, in which $\triangledown$ is a $C_q$ and $\triangle$, a $C_r$. Triangle edges correspond to edges incident to vertices in the relative subgraph, in which there is no common endpoint. Inside each of these symbols, we show the sum of the vertex weights of the corresponding sugraph.

Note that the solution must includes all vertices of the $C_{105}$ cycles and at most vertices of $3$ subgraphs $P_{13}$. Thereby, there are three possibilities that corresponds to the {\sc Steiner Tree} solutions $G[\{ a,c,d,e \}]$, $(G[\{a,b,c,d\}] - ab)$ and $(G[\{a,b,c,d\}] - bc)$.

\subsection{Polynomial-time reduction from {\sc Weighted Connected Subgraph}}\label{sec:1-disc}

In this section, we show a reduction from \pname{Weighted Connected Subgraph}. This reduction can be used to prove {\NPcness} for \pname{Weighted Connected Matching} for bipartite and planar graphs. However, we ended up having stronger results for these two classes, as its weights can be bounded to two values. This proofs will be presented in Theorems \textcolor{red}{...}.

Although we could not find any relevant use of this reduction for now, it can remain as part of future {\NPcness} proofs for \pname{Weighted Connected Matching}. Since the reduction makes minor changes to the \pname{Weighted Connected Subgraph} input graph, most of its properties should be preserved. So, if any other graph class is proven to be {\NPc} for \pname{Weighted Connected Subgraph}, it is mostly likely that it is {\NPc} for \pname{Weighted Connected Matching} also.

Let $(G'=(V',E'),k')$ be an instance of {\sc Weighted Connected Subgraph }. Also, let $q$ be the sum of all the positive vertex weights of $G'$, as formally described in the following equation.

\begin{align*}
  q &= 1 + \sum_{\substack{v \in V'\\weight(v) > 0}}^{} weight(v) \\
\end{align*}

For the {\sc Weighted Connected Matching} input, we set $k = k'$ and the graph $G=(V,E)$ obtained by the following steps.

\begin{enumerate}[(I)]
    \item For each vertex $w \in V'$, add to $G$ a copy of $K_2$, whose vertices are labeled $v_w$ and $u_w$. Besides, the edge $v_wu_w$ is such that $weight(v_wu_w)$ of $G$ equals $weight(w)$ of $G'$.
    \item For each edge of $E'$, whose endpoints are $x$ and $y$, add to $G$ the edge $v_xv_y$ and set $weight(v_xv_y) = -q$.
\end{enumerate}

In this transformation, we make an equivalence between finding a weighted connected matching in $G$ and a weighted connected subgraph in $G'$. We build the graph $G$ in such way that the only possible saturated edges are those in $\{ v_xu_x | x \in G' \}$. This is true as we set the other edge weights to $-q$. The value $q$ is slightly greater than all the positive weights together. Thereby, setting some edge weights to $-q$ make this edges never part of the desired connected matching because it is never worth selecting them.

Therefore, by the transformation, selecting an edge $v_xu_x$ to a weighted connected matching in $G$ is equivalent to select $x$ to a weighted connected subgraph in $G'$.

Note that transforming $G'$ into $G$ does not change much of the graph structure. These two graphs share many properties in common. Thereby, we can conclude the {\NPHness} of {\sc Weighted Connected Macthing} for some classes for which {\sc Weighted Connected Subgraph} is also {\NPH}. In Lemma~\ref{lemma:wcm-properties}, we present some if these properties that are interesting to our proof.

\begin{comment}
\begin{lemma}\label{lemma:wcm-properties}
Let $G'=(V',E')$ be any input graph for {\sc Weighted Connected Subgraph} and $G=(V,E)$ its transformation graph for {\sc Weighted Connected Matching}, as described below. Then, $\delta(G) = \delta(G'+1)$, $\Delta(G) = \Delta(G') + 1$ and, if $G'$ is planar or bipartite, so $G$ has also the same properties.
\end{lemma}

\begin{proof}
First we show that the diameter of $G$, $\delta(G)$, equals $\delta(G'+1)$. This can be concluded if we compare $G'$ to $G$. As $G'$ is exactly the same graph as $G'[P]$, considering $P = \{ v_w | w \in V' \}$. The graph $G$ is this exact graph, with the addition of the vertices $u_w$, $w \in V'$, whose degree is $1$. The remaining vertices, $\{ v_w | w \in V' \}$ have the same degree as $w$ in $G'$ plus $1$, because of the edge $v_wu_w$. This also reflects in the maximum vertex degree, which respects the equality $\Delta(G) = \Delta(G') + 1$.

If $G'=(V_1' \dot{\cup} V_2', E')$ is bipartite, then $G=(V_1 \dot{\cup} V_2, E)$ is also bipartite, as we can build the two bipartitions of $G$ as follows. If $w \in V'_1$, then add $v_w$ to $V_1$ and $u_w$ to $V_2$. Otherwise, add $v_w$ to $V_2$ and $u_w$ to $V_1$.

Also, we observe that $G$ in comparison to $G'$ have only one more new vertex connected to each vertex of $G'$. Then, if $G'$ is planar, then $G$ is also planar.
\end{proof}

\end{comment}



\begin{lemma}\label{lemma:wcs-1-ida}
Let $(G',k)$ be an input of {\sc Weighted Connected Subgraph }, $V'$ be a solution of this instance, and $G$ be the transformation graph obtained from this input. A connected matching $M$ in $G$ whose weight is at least $k$ can be obtained in polynomial time.
\end{lemma}
\begin{proof}
\textcolor{red}{TODO}
\end{proof}

\begin{lemma}\label{lemma:wcs-1-volta}
Let $(G',k)$ be an input of {\sc Weighted Connected Subgraph }, $G$ be the transformation graph obtained from this input and $M$ a connected matching in $G$ whose weight is at least $k$. A solution $V'$ for this {\sc Weighted Connected Subgraph } instance can be obtained in polynomial time.
\end{lemma}
\begin{proof}
\textcolor{red}{TODO}
\end{proof}

Based on Lemmas~\ref{lemma:wcs-1-ida} and \ref{lemma:wcs-1-vvolta}, we conclude this reduction with Theorem~\ref{theo:wcs-to-wcm}.

\begin{theorem}\label{theo:wcs-to-wcm}
{\sc Weighted Connected Subgraph} has a polynomial-time reduction to {\sc Weighted Connected Matching}
\end{theorem}

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{images/emp-conexo-pond-red-3-example.png}
    \caption{Example of an input graph for the {\sc Weighted Connected Subgraph}}
    \label{fig:wcs-red-3-1}
\end{figure}

\subsection{Example}

We consider the input for {\sc Weighted Connected Subgraph} as $k = 17$ and the graph as illustrated in Figure~\ref{fig:wcs-red-3-1}. In this instance, the $q$ assumes $1+ weight(a) + weight(b) + weight(d) + weight(e) + weight(h) = 1+6+2+6+4+5 = 24$.

The transformation input graph $G$ for {\sc Weighted Connected Matching} is illustrated in Figure~\ref{fig:wcs-red-3-2}. Note that, for every vertex $x$ in $G'$, there are, in $G$, two adjacent vertices $v_x$ and $u_x$ such that $weight(v_xu_x)$ equals $weight(x)$ in $G'$. All the remaining edges will have its weights set to $-q = -24$.

For example, the vertex $d$ in $G'$ corresponds to the vertices $v_d$ and $u_d$ in $G$, that are connected by an edge whose weight is $6$. Also, vertices $b$ and $f$ are adjacent in $G'$ and, so, there is an edge $v_bv_f$ in $G$ whose weight is $-24$.

In this instance, the solution for {\sc Weighted Connected Matching} is the matching $\{ u_av_a, u_bv_b, u_cv_c, u_dv_d, u_ev_e \}$. This corresponds to the {\sc Weighted Connected Subgraph} solution $\{ a,b,c,d,e \}$. Both solutions are represented in bold in Figures~\ref{fig:wcs-red-3-1} and~\ref{fig:wcs-red-3-2}


\begin{figure}
    \centering
    \includesvg[width=1\textwidth]{images/svg/emp-conexo-pond-red-3-example-2}
    \caption{Example of a reduction graph for {\sc Weighted Connected Matching}}
    \label{fig:wcs-red-3-2}
\end{figure}
